The Fairness of Leximin in Allocation of Indivisible Chores

The leximin solution -- which selects an allocation that maximizes the minimum utility, then the second minimum utility, and so forth -- is known to provide EFX (envy-free up to any good) fairness guarantee in some contexts when allocating indivisible goods. However, it remains unknown how fair the leximin solution is when used to allocate indivisible chores. In this paper, we demonstrate that the leximin solution can be modified to also provide compelling fairness guarantees for the allocation of indivisible chores. First, we generalize the definition of the leximin solution. Then, we show that the leximin solution finds a PROP1 (proportional up to one good) and PO (Pareto-optimal) allocation for 3 or 4 agents in the context of chores allocation with additive distinct valuations. Additionally, we prove that the leximin solution is EFX for combinations of goods and chores for agents with general but identical valuations.

==> acknowledgement.tex <==
\section{Acknowledgement}
We would like to thank Dr. Kamesh Munagala for bringing this topic to our attention, for providing generous advice and help through
out the project, for guiding us into this field and for counseling us with priceless life wisdom. 


==> aversion.tex <==
\section{The aversion function}
For allocation of goods, we have valuation function $v_i(\cdot)$ that depicts the utility of goods to agent $i$. This valuation function is required to be non-negative. However, for allocation of chores, the valuation function $v_i(\cdot)$ is non-positive, making it less easy to reason about. Therefore, in problems that involve only chores, we define the aversion function
$$u_i(\cdot) = |v_i(\cdot)|$$
In this way, $u_i(\cdot)$ is a non-negative function that depicts agent $i$'s aversion toward the chores. We also modify the definition of EF1 and PROP1 for $u_i(\cdot)$.
\begin{definition}[EF1 for chores]
An allocation $A$ is envy-free up to one item (EF1) if for all $i,j \in \mathcal{N}$, either $u_i(A_i) \leq u_i(A_j)$ or $\exists c \in A_i$ s.t. $u_i(A_i) \leq u_i(A_j\cup\{c\})$.
\end{definition}
\noindent Note again $u_i(A_i) \leq u_i(A_j\cup\{c\})$ is equivalent to $u_i(A_i\backslash\{c\}) \leq u_i(A_j)$ for additive utilities.
\begin{definition}[PROP1 for chores]
An allocation $A$ is proportional up to one item (PROP1) if for all $i\in\mathcal{N}$, either $u_i(A_i) \leq u_i(\mathcal{M})/n$ or $\exists c \in A_i$ s.t. $u_i(A_i\backslash\{c\}) \leq u_i(\mathcal{M})/n$.
\end{definition}

==> efficient.tex <==
\section{Efficient algorithm for identical additive valuations}
\label{sec:efficient}
In the case of identical additive valuations, any allocation is PO. In \cite{barman2018greedy}, Barman \etal gave an algorithm, which they call ALG-IDENTICAL, that finds an EFX allocation of goods in polynomial time. In this section we show that a modification to ALG-IDENTICAL can find EFX allocations for combinations of goods and chores. Our modified ALG-IDENTICAL is shown in Algorithm \ref{alg:identical}. If an item $o$ has valuation $v(o)=0$, we define it as a good.
\begin{algorithm}
\caption{ALG-IDENTICAL}
\label{alg:identical}
\begin{algorithmic}
	\STATE Order the items in decreasing order of absolute value, i.e., $|v(o_1)| \geq |v(o_2)| \geq \ldots \geq |v(o_m)|$.
	\STATE Set $A \leftarrow (\emptyset, \ldots, \emptyset)$
	\FOR{$l \in \{1, \dots, m\}$}
	\IF{$v(o_l) \geq 0$}
	\STATE $i \leftarrow \argmin_{k\in\mathcal{N}} v(A_k)$
	\ELSE
	\STATE $i \leftarrow \argmax_{k\in\mathcal{N}} v(A_k)$
	\ENDIF
	\STATE $A_i \leftarrow A_i\cup\{o_l\}$
	\ENDFOR
	\RETURN $A$
\end{algorithmic}	
\end{algorithm}

\begin{theorem}
For identical additive valuations, the allocation $A$ returned by ALG-IDENTICAL is EFX.
\end{theorem}
\begin{proof}
Let $A^l$ be the allocation maintained by ALG-IDENTICAL at the end of the $l$th iteration. $A^0 = (\emptyset, \dots, \emptyset)$. It suffices to show that for $l\in\{1,\dots,m\}$, if $A^{l-1}$ is EFX, then so is $A^l$. Consider the following two cases. \\~\\
\textbf{Case 1: $v(o_l) \geq 0$.} In this case $o_l$ is assigned to agent $i \in \argmin_{k\in\mathcal{N}} v(A^{l-1}_k)$, so $A_i^l = A_i^{l-1}\cup\{o_l\}$ and $A_j^l = A_j^{l-1}\ \forall j \neq i$. Since agent $i$ is allocated one more good, agent $i$ will stay at least EFX to all other agents. If $v(A^l_j) \geq v(A^l_i)\ \forall j \in \mathcal{N}$, we are done since no other agent envies agent $i$. If there exists agent $j$ such that $v(A^l_j) < v(A^l_i)$, we must also have $v(A^{l-1}_i) = v(A^l_i) - v(o_l) \leq v(A^l_j)$ from how we chose agent $i$. Recall that we order the items in decreasing order of absolute value, so all items $o$ that have been assigned have $|v(o)| \geq v(o_l)$. Therefore, if we remove any good from agent $i$'s bundle or any chore from agent $j$'s bundle, agent $j$ will not envy agent $i$ anymore, and $A^l$ is still EFX. \\~\\
\textbf{Case 2: $v(o_l) < 0$.} In this case $o_l$ is assigned to agent $i \in \argmax_{k\in\mathcal{N}} v(A^{l-1}_k)$, so $A_i^l = A_i^{l-1}\cup\{o_l\}$ and $A_j^l = A_j^{l-1}\ \forall j \neq i$. Since agent $i$ is allocated one more chore, all other agent $j$ will stay at least EFX to agent $i$. If $v(A^l_i) \geq v(A^l_j)\ \forall j \in \mathcal{N}$, we are done since agent $i$ does not envy any other agent. If there exists agent $j$ such that $v(A^l_i) < v(A^l_j)$, we must also have $v(A^l_j)  \leq v(A^l_i) + |v(o_l)| = v(A^{l-1}_i)$. Recall that we order the items in decreasing order of absolute value, so all items $o$ that have been assigned have $|v(o)| \geq |v(o_l)|$. Therefore, if we remove any good from agent $j$'s bundle or any chore from agent $i$'s bundle, agent $i$ will not envy agent $j$ anymore, and $A^l$ is still EFX.
\end{proof}

==> mnw.tex <==
\section{Challenges with chores allocation}
\label{sec:mnwfailure}
Aziz noted in \cite{Aziz2016ComputationalSC} that in problems involving more than two agents, results for goods allocation do not necessarily carry over to chores allocation. Here we show two failed attempts to adapt the MNW solution to chores allocation. \\

\noindent The original MNW solution, which achieves both EF1 and PO in goods allocation with additive valuations, is defined as follows \cite{Caragiannis2016TheUF}.
\begin{definition}
The Nash welfare of an allocation $A$ is defined as $NW(A) = \prod_{i \in \mathcal{N}} v_i(A_i)$. The MNW solution selects an allocation $A^{MNW}$ that maximizes the modified Nash welfare among all feasible allocations, i.e.
$$A^{MNW} \in \argmax_{A \in \Pi_n (\mathcal{M})} NW(A).$$
\end{definition}
\noindent The natural question arising as we start to look at this problem is whether we could adapt this elegant and powerful MNW solution to the context of chores allocation. Unfortunately, both our attempts failed miserably.\\~\\ 
\noindent Our first attempt is simple and intuitive. Here we treat the chores that are not included in each agent's bundle as her "utility". Based on this intution, we come up with the following modified Maximum Nash Welfare solution.
\begin{definition}
The modified Nash welfare of an allocation $A$ is defined as $NW'(A) = \prod_{i \in \mathcal{N}} [u_i(\mathcal{M}) - u_i(A_i)]$. The modified maximum Nash welfare (MNW') solution selects an allocation $A^{MNW'}$ that maximizes the modified Nash welfare among all complete allocations, i.e.
$$A^{MNW'} \in \argmax_{A \in \Pi_n (\mathcal{M})} NW'(A).$$
\end{definition}

\noindent However, consider the example in Table \ref{tab:mnw}, where the MNW' solution is marked by the circles. This allocation is not PROP1 because $u_1(A_1\backslash\{c\})=12 > u_1(\mathcal{M})/3=11\ \forall c\in A_1=\{a,b,c\}$. In other words, this MNW' solution even fails to guarantee PROP1 in chores allocation.
\begin{table}[h]
    \centering
    \begin{tabular}{|c||c|c|c|c|c|}
        \hline
         & a & b & c & d & e \\ \hline \hline
         Agent 1 & \circled{6} & \circled{6} & \circled{6} & 7 & 8 \\ \hline
         Agent 2 & 10 & 10 & 10 & \circled{1} & 2 \\ \hline
         Agent 3 & 10 & 10 & 10 & 2 & \circled{1} \\ \hline
        \end{tabular}
    \caption{An example where the modified MNW solution fails to achieve PROP1}
    \label{tab:mnw}
\end{table}
\noindent Our second attempt is inspired by the result of Bogomolnaia \etal in \cite{bogomolnaia2017competitive}. They showed that for divisible chores, the efficient allocation that maximizes $\prod_{i\in\mathcal{N}} u_i(A_i)$ guarantees EF and PO. We seek this exact same solution subject to indivisibility and call it the constrained MNW solution as we only consider efficient allocations. \\However, consider the two examples in Table \ref{tab:mnw2} and \ref{tab:mnw3}, where the constrained MNW solutions are marked by the circles. In Table \ref{tab:mnw2} with 3 agents, the allocation is not EF1 because $u_1(A_1\setminus\{c\}) \geq 5 > u_1(A_2) = 3\ \forall c\in A_1$. In Table \ref{tab:mnw3} with 5 agents, the allocation is not PROP1 because $u_1(A_1\setminus\{c\}) \geq 10.3 > u_1(\mathcal{M}) / 5 = 10\ \forall c \in A_1$.
\begin{table}[h]
    \centering
    \begin{tabular}{|c||c|c|c|c|c|}
        \hline
         & a & b & c & d & e \\ \hline \hline
         Agent 1 & \circled{2} & \circled{3} & \circled{3} & 3 & 9 \\ \hline
         Agent 2 & 2 & 3 & 9 & \circled{2} & 4 \\ \hline
         Agent 3 & 1 & 1 & 1 & 5 & \circled{12} \\ \hline
        \end{tabular}
    \caption{An example where the constrained MNW solution fails to achieve EF1}
    \label{tab:mnw2}
\end{table}
\begin{table}[h]
    \centering
    \begin{tabular}{|c||c|c|c|c|c|c|c|}
        \hline
         & a & b & c & d & e & f & g \\ \hline \hline
         Agent 1 & \circled{10.3} & \circled{12.2} & 10 & 2.2 & 12.7 & 1.1 & 1.5 \\ \hline
         Agent 2 & 7.9 & 9.4 & \circled{1.4} & \circled{5.7} & 7.4 & 10.3 & 7.9 \\ \hline
         Agent 3 & 9.8 & 6 & 6.5 & 9.6 & \circled{6.8} & 7.4 & 3.9 \\ \hline
         Agent 4 & 7.5 & 10.1 & 2.5 & 8.1 & 8 & \circled{6.6} & 7.2 \\ \hline
         Agent 5 & 10.5 & 6.3 & 6.4 & 1 & 6.1 & 13.7 & \circled{6} \\ \hline
        \end{tabular}
    \caption{An example where the constrained MNW solution fails to achieve PROP1}
    \label{tab:mnw3}
\end{table}~\\
We hope that these two failed attempts could motivate our readers about the potential difficulty of migrating techniques from goods allocation to chores allocation.

==> related.tex <==
\section{Related work}
Fair allocation of indivisible goods has been studied extensively in the past. Here we will only include the results that are most closely related to this paper. In the context of goods allocations, in \cite{Lipton2004OnAF}, Lipton \etal provided an algorithm that finds EF1 allocations for general valuations but does not guarantee PO. In \cite{Caragiannis2016TheUF}, Caragiannis \etal showed that the maximum Nash welfare (MNW) solution guarantees EF1 and PO for additive valuations. In \cite{Roughgarden2017AlmostEF}, Plaut and Roughgarden showed that the leximin solution guarantees EFX and PO for general but identical valuations with nonzero marginal utility. Meanwhile, the leximin++ solution guarantees EFX but not PO for all general but identical valuations. In the same paper, they also proposed a cut-and-choose-based algorithm for two agents with general and possibly distinct valuations that is guaranteed to produce an EFX allocation. \\

\noindent However, fair allocation of indivisible chores only started to receive attention after Aziz noted that the results in goods allocation with more than two agents may not necessarily carry over to chores \cite{Aziz2016ComputationalSC}. In \cite{aziz2018fair}, Aziz \etal showed that the double round robin algorithm can always generate an EF1 allocation when valuations are additive. For the two agent case, they present a polynomial-time algorithm that finds an EF1 and PO allocation. In \cite{aleks2018envy}, Aleksandrov showed that a modified version of the leximin++ solution, which he calls leximax-, finds EFX allocations for indivisible chores with anti-monotone identical valuations.
